Diverse Text Generation via Variational Encoder-Decoder Models with Gaussian Process Priors

Generating high quality texts with high diversity is important for many NLG applications, but current methods mostly focus on building deterministic models to generate higher quality texts and do not provide many options for promoting diversity. In this work, we present a novel latent structured variable model to generate high quality texts by enriching contextual representation learning of encoder-decoder models. Specifically, we introduce a stochastic function to map deterministic encoder hidden states into random context variables. The proposed stochastic function is sampled from a Gaussian process prior to (1) provide infinite number of joint Gaussian distributions of random context variables (diversity-promoting) and (2) explicitly model dependency between context variables (accurate-encoding). To address the learning challenge of Gaussian processes, we propose an efficient variational inference approach to approximate the posterior distribution of random context variables. We evaluate our method in two typical text generation tasks: paraphrase generation and text style transfer. Experimental results on benchmark datasets demonstrate that our method improves the generation quality and diversity compared with other baselines.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)
	grep -e "Warning" --color auto obj/$(PROJECT).log


==> ethical.tex <==
\section{Ethical Considerations}
% Does the paper describe the characteristics of the dataset in enough detail for a reader to understand which speaker populations the technology could be expected to work for?
% Do the claims in the paper match the experimental results, in terms of how far the results can be expected to generalize?
% Does the paper describe the steps taken to evaluate the quality of the dataset?

The goal of this work is to enrich the potential of a language model for generating diverse texts.
Key features of each dataset adopted in this paper are described in the experiment session.
To further guarantee the reproducibility of this work, we provide all the essential details in the main content and the appendices. Codes and models will also open to public after the review period.

Although this work itself does not directly involve any ethical issues, the proposed method faces the same ethical challenges as other natural language generation techniques do.
For example, in dialogue systems, diverse generation systems may produce some offensive or toxic responses. Advanced text generation models could be used in scams.
Additional efforts are needed, both in technology and in society, to alleviate these issues.
Filtering toxic words and deploying spam-detection systems are two of the many examples.

==> prior.tex <==
\section{Learning with Gaussian Process Priors}
\label{sec:model}

% \begin{itemize}
% \item motivation
% \item what is GP?
% \item why use GP?
% \item anything else?
% \end{itemize}

Intuitively, the random function $g(\vec{h}_i)$ needs to satisfy two constraints simultaneously: (1) it can introduce some randomness that allows some variations; (2) it should maintain the majority of the information in $\vec{h}_i$ in order to be a faithful representation. 
Therefore, the definition of the random function $g(\vec{h}_i)$ is the key for the proposed method to be successful. 

In this section, we start with standard attention-based Seq2Seq models, then we introduce a random function which imposes randomness in the encoder hidden states.
Finally, we propose our Gaussian process prior to learn a better random function, which not only introduces randomness into context representations, but also well preserve the semantic information.


% \note[WD]{In this section, I introduce our GP prior, and briefly state the generative story of our variational Seq2Seq framework.}


In this work, instead of giving an explicit form of $g(\vec{h}_i)$, we assign $g(\vec{h}_i)$ with a probability distribution using Gaussian process.
As shown in Figure\autoref{fig:gp-prior}, we can sample very different functions $g(\vec{h}_i)$ from the same Gaussian process prior, which ensures randomness when generating $\vec{z}_i$.



\begin{comment}
A Gaussian process prior is fully specified by a mean function $m(\cdot)$ and a covariance function $k(\cdot,\cdot)$:
\begin{equation}
  \label{eq:gp-prior}
  g(\vec{h}) \sim \mathcal{GP}(m(\vec{h}), k(\vec{h}, \vec{h}')), 
\end{equation}
where, as a prior, $m(\cdot)$ is usually a zero function and $k(\vec{h}, \vec{h}')=\mathbb{E}{[g(\vec{h})-m(\vec{h})(g(\vec{h}')-m(\vec{h}')]}$. 
The choice of $k(\cdot, \cdot)$ in a Gaussian process encodes the correlation of different $\vec{z}$'s in \autoref{eq:ssm-obs}.
Generally, given a sequence of input $\vec{x}_{1:N}$ and its corresponding hidden states $\vec{h}_{1:N}$ from the transition function, the subset of function values $\vec{z}_{1:N}$ computed via \autoref{eq:ssm-obs} are jointly Gaussian distributed:
\begin{equation}
  \begin{split}
  \label{eq:joint-prior}
    p(\vec{z}_{1:N}) = \prod_{i=1}^N \mathcal{N}(m(\vec{h}_i), k(\vec{h}_i,\vec{h}_i'))
  \end{split}
\end{equation}
where $m(\vec{h}_i)$ is the value of the prior mean function with input $\vec{h}_i$ and $k(\vec{h}_i,\vec{h}_i')$ gives the covariance between encoder hidden states at time steps $i$ and other encoding time steps.
According to the property of Gaussian processes\cite{rasmussen2006gaussian}, 
the conditional distribution of a Gaussian process is still a Gaussian process.
If we observed $\vec{z}_{1:N}$, then we can have a good estimation of the random function $g(\cdot)$ conditioned on $\vec{z}_{1:N}$, which is still a Gaussian process
\begin{equation}
  \label{eq:post}
  g(\cdot)\mid \vec{z}_{1:N} \sim \mathcal{GP}(\vec{\eta}(\cdot), \vec{u}(\cdot,\cdot))
\end{equation}
with
\begin{equation}
  \begin{split}
    \label{eq:cov}
    \vec{\eta}(\cdot) &= {m}(\cdot) + k(\cdot, \mat{H})\mat{K}^{-1}(\vec{z}-\vec{m})\\
    \vec{u}(\cdot,\cdot) &= k(\cdot, \cdot) - k(\cdot, \mat{H})\mat{K}^{-1} k^\top(\cdot, \mat{H})
  \end{split}
\end{equation}
Theoretically, \autoref{eq:post}
can be used on any given $\vec{h}$.
Therefore, it is also called the predictive distribution in the literature of Gaussian process \cite{rasmussen2006gaussian,deisenroth2011robust,frigola2014variational,eleftheriadis2017identification}.
Given $\vec{z}_i$ as latent state for the encoder hidden state $\vec{h}_i$, and the mapping function $\vec{z}_i=g(\vec{h}_i)+\epsilon_g$ with Gaussian random noise $\epsilon_g \sim \mathcal{N}(\vec{0}, \sigma_g^2 \mat{I})$.
\end{comment}

Specifically, in this work, we use a Gaussian process defined with a 
In order to preserve the majority of the information in $\vec{h}_{1:N}$, we introduce a specific Gaussian process prior for the mapping function $g(\vec{h}_i)$:
\begin{equation}
\begin{split}
\label{eq:gp-ours}
    g(\vec{h}) &\sim \mathcal{GP}(m(\vec{h}), k(\vec{h}, \vec{h}'))\\
    m(\vec{h}_i) &= f(\vec{h}_{i-1}, \vec{x}_i) \\
    k(\vec{h}_i, \vec{h}_j) &= 
    v^2 \exp\{-\frac{1}{2}\sum_{d=1}^D(\frac{|\vec{h}^{(d)}_{i} - \vec{h}^{(d)}_j|}{r})^2\} 
\end{split}
\end{equation}
We use a mean function $m(\vec{h}_i)=\vec{h}_i$ for our Gaussian process prior.
The interpretation for this mean function is that when we have not observed any training data $\mathcal{D}$, we assume all possible function values $g(\vec{h}_i)$ are centered around $\vec{h}_i$, which enables us to introduce random perturbation on the encoder hidden state $\vec{h}_i$.
The covariance function $k$ is a squared exponential function, where $\{v, r\}$ is a set of hyper-parameters used to control the signal variance and length scale of the covariance function, and $d$ is the dimension index of the encoder hidden state. The squared exponential function is widely used as a linear smoother to reconstruct the underlying signal $g(\vec{h}_i)$ by removing the noise $\epsilon_i$.


When predicting the output sentence $\vec{y}_{1:T}$, we first sample a function $g$ from our Gaussian process prior, then sample the latent context variables $\vec{z}_{1:N}$ conditioning on function values computed from that sampled function $g$, finally predict the output sentence $\vec{y}_{1:T}$ based on the sampled latent context variables $\vec{z}_{1:N}$.
The overall generative process for our variational Seq2Seq framework is demonstrated in \autoref{alg:generative}.

Note that the standard variational Seq2Seq model \cite{bowman2016generating} with a standard Gaussian prior $p(\vec{z})=\mathcal{N}(\vec{0}, \mat{I})$  is a special case under our variational Seq2Seq framework.
In this case, the mapping function $g$ always maps the encoder hidden state $\vec{h}_i$ into zero mean with variance equals to one.

\input{alg}

==> tab/dia-sents.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{lp{0.45\textwidth}|p{0.45\textwidth}}
    \toprule
     \multicolumn{3}{p{0.95\textwidth}}{\textit{Context}: \textcolor{red}{User0}: are you free this weekend , miss rose ? \underline{\hspace{0.4cm}}eou\underline{\hspace{0.4cm}} 
     \textcolor{blue}{User1}: yes , i am . what 's up ? \underline{\hspace{0.4cm}}eou\underline{\hspace{0.4cm}} 
     \textcolor{red}{User0}: then would you please go to a dance party with me ? \underline{\hspace{0.4cm}}eou\underline{\hspace{0.4cm}} 
     \textcolor{blue}{User1}: with pleasure . i suppose you dance often .
     } \\
     \multicolumn{3}{p{0.95\textwidth}}{\textit{Reference}: \textcolor{red}{User0}: oh , no . as a matter of fact , i have n't danced for a long time .} \\
    \midrule
    & \textbf{VHRED} & \textbf{Attn-Seq2Seq + GP Prior (Ours)} \\
    [0.3em]
    1 & \textcolor{red}{User0}: oh , yes . i like the best man . i love it very much .& \textcolor{red}{User0}: i am not sure , but you know , i am a great dancer. \\
    2 & \textcolor{red}{User0}: oh , yes . i think that 's a good idea . & \textcolor{red}{User0}: no , i 'm not too busy . i 'm not sure of that .\\
    3 & \textcolor{red}{User0}: oh , yes . i like the best man . the music is really good at the same music . & \textcolor{red}{User0}: i am not sure , but you know i 'm not much of a dancer .\\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:z-daily}
    Sample outputs conditioned on different $\vec{z}_{1:N}$ sampled from $q_{\vphi}(\vec{z}\mid \vec{h}, \vec{y})$ on DailyDialog test set.
  }
\end{table*}

==> tab/dialog.tex <==
\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lllll}
    \toprule
    Methods & BLEU & METEOR & Dist-1 & Dist-2 \\
    \midrule 
    Attn-Seq2Seq & 0.111 & 0.109 & 0.026 & 0.131 \\
    HRED & 0.100 & 0.104 & 0.019 & 0.091 \\
    VHRED & 0.101 & 0.105 & 0.023 & 0.105 \\
    Our GP Prior & 0.107 & 0.108 & \textbf{0.027} & \textbf{0.131} \\
    Our GP Prior$^\dagger$ & \textbf{0.117} & \textbf{0.113} & 0.024 & 0.113 \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:dialog-acc}
  Model performance on DailyDialog test set. 
  Our GP Prior$^\dagger$ is the results after oracle-ranking.}
\end{table}
